Evaluating Disentanglement of Structured Representations

We introduce the first metric for evaluating disentanglement at individual hierarchy levels of a structured latent representation. Applied to object-centric generative models, this offers a systematic, unified approach to evaluating (i) object separation between latent slots (ii) disentanglement of object properties inside individual slots (iii) disentanglement of intrinsic and extrinsic object properties. We theoretically show that for structured representations, our framework gives stronger guarantees of selecting a good model than previous disentanglement metrics. Experimentally, we demonstrate that viewing object compositionality as a disentanglement problem addresses several issues with prior visual metrics of object separation. As a core technical component, we present the first representation probing algorithm handling slot permutation invariance.

==> figures/overview_debug.tex <==

\begin{figure}[b]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tikzpicture}[
 scale = 1,
 arrow/.style = {thick,-stealth},
 mydashed/.style={dashed,dash phase=3pt}
 ]
 
% MATRIX 1
 \matrix[matrix of math nodes,nodes={align=center, text width=1cm,text depth=0.3cm},left delimiter={(},right delimiter={)},ampersand replacement=\&] (mat1) {
    R_{1,1}\& R_{1,2} \& R_{1,3}\& R_{1,4} \\ 
    R_{2,1}\& R_{2,2} \& R_{2,3}\& R_{2,4} \\ 
    R_{3,1}\& R_{3,2} \& R_{3,3}\& R_{3,4} \\ 
    R_{4,1}\& R_{4,2} \& R_{4,3}\& R_{4,4} \\ 
 };
 
\draw[color=blue, ultra thick,dashed] ($ (mat1-1-1.south west) + (0.1,0.2) $) rectangle ($ (mat1-1-1.north east) + (-0.1,0) $);
\draw[color=blue, ultra thick] ($ (mat1-1-2.south west) + (0.1,0.2) $) rectangle ($ (mat1-1-2.north east) + (-0.1,0) $);
\draw[color=blue, ultra thick] ($ (mat1-2-1.south west) + (0.1,0.2) $) rectangle ($ (mat1-2-1.north east) + (-0.1,0) $);
\draw[color=blue, ultra thick] ($ (mat1-2-2.south west) + (0.1,0.2) $) rectangle ($ (mat1-2-2.north east) + (-0.1,0) $);

\draw[color=red, ultra thick, mydashed] ($ (mat1-1-1.south west) + (0.1,0.2) $) rectangle ($ (mat1-1-1.north east) + (-0.1,0) $);
\draw[color=red, ultra thick] ($ (mat1-1-3.south west) + (0.1,0.2) $) rectangle ($ (mat1-1-3.north east) + (-0.1,0) $);
\draw[color=red, ultra thick] ($ (mat1-3-1.south west) + (0.1,0.2) $) rectangle ($ (mat1-3-1.north east) + (-0.1,0) $);
\draw[color=red, ultra thick] ($ (mat1-3-3.south west) + (0.1,0.2) $) rectangle ($ (mat1-3-3.north east) + (-0.1,0) $);

% FACTORS
% Groups
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat1.north west) + (0,0.3) $)  -- ($ (mat1.126) + (0,0.3) $) node (mat1color1) [midway, above=0.5em] {Color};
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat1.123) + (0,0.3) $)  -- ($ (mat1.92) + (0,0.3) $) node (mat1or1) [midway, above=0.5em] {Size};

\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat1.88) + (0,0.3) $)  -- ($ (mat1.55) + (0,0.3) $) node (mat1color2) [midway, above=0.5em] {Color};
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat1.52) + (0,0.3) $)  -- ($ (mat1.north east) + (0,0.3) $) node (mat1or2) [midway, above=0.5em] {Size};

% Components
\draw[decorate, decoration ={brace,raise=1pt}] (mat1color1.north west) -- (mat1or1.north east) node (mat1obj1) [midway, above=0.5em] {Object 1};
\draw[decorate, decoration ={brace,raise=1pt}] (mat1color2.north west) -- (mat1or2.north east) node (mat1obj2) [midway, above=0.5em] {Object 2};

% All
\draw[decorate, decoration ={brace,raise=1pt}] (mat1obj1.north west) -- (mat1obj2.north east) node (mat1gt) [midway, above=0.5em] {Factors of variation};

% LATENTS
% Dimensions
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat1.south west) + (-0.3,0) $)  -- ($ (mat1.200) + (-0.3,0) $) node (mat1dim4) [midway, left=1em] {Dim 2};
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat1.198) + (-0.3,0) $)  -- ($ (mat1.181) + (-0.3,0) $) node (mat1dim3) [midway, left=1em] {Dim 1};
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat1.179) + (-0.3,0) $)  -- ($ (mat1.163) + (-0.3,0) $) node (mat1dim2) [midway, left=1em] {Dim 2};
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat1.160) + (-0.3,0) $)  -- ($ (mat1.north west) + (-0.3,0) $) node (mat1dim1) [midway, left=1em] {Dim 1};
 
 
% Slots 
\draw[decorate, decoration ={brace,raise=1pt}] (mat1dim2.south west) -- (mat1dim1.north west) node (mat1slot1) [midway, left=0.5em] {Slot 1};
\draw[decorate, decoration ={brace,raise=1pt}] (mat1dim4.south west) -- (mat1dim3.north west) node (mat1slot2) [midway, left=0.5em] {Slot 2};

% ALl
\draw[decorate, decoration ={brace,raise=1pt}] (mat1slot2.south west) -- (mat1slot1.north west) node (mat1lat) [midway, left=0.5em] {Latents};







% MATRIX 2
 
 \matrix[matrix of nodes,nodes={align=center, text width=2cm,text depth=1cm},left delimiter={(},right delimiter={)},below=5em of mat1,,ampersand replacement=\&] (mat2) {
    {$R_{1,1} +  R_{1,2} +$\\ $R_{2,1} + R_{2,2}$} \& {$R_{1,3} + R_{1,4}$ +\\ $R_{2,3} + R_{2,4}$}  \\ 
    {$R_{3,1} +  R_{3,2} +$\\ $R_{4,1} + R_{4,2}$} \& {$R_{3,3} + R_{3,4} +$\\ $R_{4,3} + R_{4,4} $} \\
 };
 
 
 
% Groups
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat2.north west) + (0,0.3) $)  -- ($ (mat2.north) + (-0.1,0.3) $) node (mat1color1) [midway, above=0.5em] {Object 1};
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat2.north) + (0.1,0.3) $)  -- ($ (mat2.north east) + (0,0.3) $) node (mat1or1) [midway, above=0.5em] {Object 2};

\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat2.south west) + (-0.3,0) $)  -- ($ (mat2.west) + (-0.3,-0.1) $) node (mat2comp1) [midway, left=0.5em] {Slot 2};
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat2.west) + (-0.3,0.1) $)  -- ($ (mat2.north west) + (-0.3,0) $) node (mat2comp2) [midway, left=0.5em] {Slot 1};
 
\draw[color=blue, ultra thick] (mat2-1-1.200) rectangle (mat2-1-1.north east);
 
 
 
% MATRIX 3
  \matrix[matrix of nodes,nodes={align=center, text width=2cm,text depth=1cm},left delimiter={(},right delimiter={)},right=8em of mat1,,ampersand replacement=\&] (mat3) {
    {$R_{1,1} +  R_{1,3} +$\\ $R_{3,1} + R_{3,3}$} \& {$R_{1,2} + R_{1,4}$ +\\ $R_{3,2} + R_{3,4}$}  \\ 
    {$R_{2,1} +  R_{2,3} +$\\ $R_{4,1} + R_{4,3}$} \& {$R_{2,2} + R_{2,4} +$\\ $R_{4,2} + R_{4,4} $} \\
 };
 

\draw[color=red, ultra thick] (mat3-1-1.200) rectangle (mat3-1-1.north east);

 
% Groups
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat3.north west) + (0,0.3) $)  -- ($ (mat3.north) + (-0.1,0.3) $) node (mat1color1) [midway, above=0.5em] {Color};
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat3.north) + (0.1,0.3) $)  -- ($ (mat3.north east) + (0,0.3) $) node (mat1or1) [midway, above=0.5em] {Size};


\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat3.south west) + (-0.3,0) $)  -- ($ (mat3.west) + (-0.3,-0.1) $) node (mat3gr1) [midway, left=0.5em] {Dim 2};
\draw[decorate, decoration ={brace,raise=1pt}] ($ (mat3.west) + (-0.3,0.1) $)  -- ($ (mat3.north west) + (-0.3,0) $) node (mat3gr2) [midway, left=0.5em] {Dim 1};
 
 
% INTER MATRIX ARROWS
\draw[color=blue,arrow, ultra thick, bend angle=45, bend right] (mat1.south west) to  node[left=0.5em,text width=2.5cm,align=center,color=blue!80!black,font=\normalsize] (proj1) {Projection on\\ slot/object}  (mat2.north west);
 
\draw[color=red,arrow, ultra thick, bend angle=45, bend left] (mat1.north east) to node[above=0.5em,text width=2.8cm,align=center,color=red!80!black,font=\normalsize] (proj2) {Projection on \\ dimension/property} (mat3.north west) ;
 
% Entropies
\draw[dashed, ultra thick] ($ (mat3-2-1.south west) + (-0.1,0.4) $) rectangle ($ (mat3-1-1.north east) + (0.1,0.2) $) node (rec1) {};
\draw[dashed, ultra thick] ($ (mat2-1-1.south west) + (-0.1,0.2) $) rectangle ($ (mat2-1-2.north east) + (0.1,0.2) $) node (rec2) {};


\draw ($ (rec2.east) + (2.3,-0.7) $) node[align=center] (dis) {Object-level\\ disentanglement};
\draw ($ (rec1.south) + (-1.2,-4) $) node[align=center] (comp) {Property-level\\ completeness};

\draw[arrow, ultra thick] ($ (rec2.east) + (0,-0.7) $) to   (dis.west);
\draw[arrow, ultra thick] ($ (rec1.south) + (-1.2,-2.7) $) to   (comp.north);

\end{tikzpicture}
}

\caption{Overview of projections on a toy example of object-centric representation. First, the affinity scores are marginalized according to the selected hierarchy level. Then,  the row (resp. column) entropy yields a measure of disentanglement (resp. completeness) in projected space.}
\label{overview}
\end{figure} 

==> tables/ablation_alg_1.tex <==
\begin{table*}[t]
\caption{Ablation study of Algorithms 1  and 2 for Multi-dSprites. We report mean and std error over three random seeds. All values are in $\%$. $100$ is the best possible score and $0$ the worst, except for the informativeness metric where $0$ is best. All models are trained with variational loss.}\label{tab_abl}
\begin{center}
\begin{footnotesize}
\begin{sc}
\tra{1.3}
\center
\addtolength{\tabcolsep}{-1pt}
\begin{tabular}{l l  c c c c c c c c c  }
\toprule
  &  \multicolumn{2}{c}{Object-level} &  & \multicolumn{2}{c}{Property-level} &\\ 
 \cline{2-3}\cline{5-6}  
 Model  &   Dis. $(\uparrow)$& Comp. $(\uparrow)$ &  & Dis.$(\uparrow)$ & Comp.$(\uparrow)$ &  Inf.$(\downarrow$) \\
\midrule
%\footnotesize \textbf{Statistic} \\
Monet (Engelcke)&     $52\pm4$ & $52\pm4$ && $39\pm6$ & $60\pm5$ & $45\pm3$ \\
Monet (Engelcke) (without Alg 1) &  $30\pm2$ & $30\pm2$ && $27\pm4$ & $53\pm3$& $51\pm3$ \\
Monet (Engelcke) (without Alg 2) &  $57\pm1$ & $57\pm1$ && $52\pm5$ & $69\pm4$& $40\pm3$ \\
 Monet (Engelcke) (without Alg 1 and 2) &  $22\pm0.5$ & $22\pm0.5$ && $9\pm1$ & $41\pm0.9$& $90\pm0.5$ \\
\midrule
Monet  &     $75\pm7$ & $75\pm7$ && $59\pm6$ & $74\pm5$ & $26\pm6$\\
Monet (without Alg 1) &     $40\pm3$ & $40\pm4$ && $44\pm5$ & $65\pm3$ & $30\pm6$\\
Monet (without Alg 2) &     $64\pm4$ & $64\pm4$ && $70\pm5$ & $79\pm3$ & $31\pm4$\\
Monet (without Alg 1 and 2) &     $24\pm1$ & $24\pm1$ && $11\pm0.8$ & $43\pm0.4$ & $88\pm0.8$\\
\midrule
Genesis	& $90\pm0.8$    & $91\pm0.6$&& $72\pm0.5$& $60\pm0.4$&$24\pm0.4$\\
Genesis (without Alg 1)& $89\pm0.1$         & $90\pm0.1$ && $72\pm0.1$ & $60\pm0.3$ & $23\pm0.4$\\
Genesis (without Alg 2)& $61\pm0.4$         & $61\pm0.4$ && $75\pm1$ & $62\pm2$ & $40\pm0.6$\\
Genesis (without Alg 1 and 2)& $33\pm0.3$         & $33\pm0.3$ && $18\pm0.3$ & $14\pm0.2$ & $89\pm0.2$\\
\midrule
 Iodine    &  $70\pm9$  & $72\pm10$  & & $37\pm5$ & $ 62\pm4$ &$37\pm6$  \\
 Iodine (without Alg 1)   & $32\pm2$         & $33\pm2$ && $21\pm1$ & $52\pm1$ & $47\pm4$\\
 Iodine (without Alg 2)   & $66\pm1$         & $66\pm1$ && $56\pm0.6$ & $72\pm0.4$ & $36\pm2$\\
 Iodine (without Alg 1 and 2)   & $26\pm0.9$         & $26\pm0.9$ && $3.8\pm0.2$ & $39\pm0.1$ & $92\pm0.3$\\
\bottomrule
\end{tabular}
\end{sc}
\end{footnotesize}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/global_comparison.tex <==
\begin{table*}[t]
\caption{Comparison of the different models on Multi-dSprites and CLEVR6. We report mean and standard error over three random seeds. All values are in $\%$. $100$ is the best possible score and $0$ the worst, except for the informativeness metric where $0$ is best. Models denoted with (R) are trained with pure reconstruction loss.}\label{tab_global}
\begin{center}
\begin{footnotesize}
\begin{sc}
\tra{1.3}
\center
\addtolength{\tabcolsep}{-1pt}
\begin{tabular}{l l  c c c c c c c c c c c }
\toprule
 & &  \multicolumn{2}{c}{Object-level} &  & \multicolumn{2}{c}{Property-level} &\\ 
 \cline{3-4}\cline{6-7}  
& Model  &   Dis. $(\uparrow)$& Comp. $(\uparrow)$ &  & Dis.$(\uparrow)$ & Comp.$(\uparrow)$ &  Inf.$(\downarrow$) & ARI$(\uparrow)$ & mSC $(\uparrow)$\\
\midrule
%\footnotesize \textbf{Statistic} \\
\multirow{7}{*}{MdSpr.}&Monet (Att.)&     $52\pm4$ & $52\pm4$ && $39\pm6$ & $60\pm5$ & $45\pm3$& $95\pm 1$ & $\bm{83 \pm0.3}$\\
& Monet (Att.) (R) &  $60\pm4$ & $60\pm4$ && $29\pm3$ & $52\pm1$& $36\pm2$ & $\bm{98\pm0.1}$ & $\bm{86\pm4}$\\
&Monet (Dec.) &     $75\pm7$ & $75\pm7$ && $59\pm6$ & $\bm{74\pm5}$ & $26\pm6$& $80\pm 4$ & $68 \pm2$\\
&Monet (Dec.) (R) &     $69\pm0.3$ & $69\pm0.2$ && $35\pm1$ & $55\pm1$ & $32\pm0.8$& $91\pm 0.2$ & $69 \pm2$\\
&Genesis	& $\bm{90\pm0.8}$    & $\bm{91\pm0.6}$&& $\bm{72\pm0.5}$& $60\pm0.4$&$\bm{24\pm0.4}$&$85\pm 0$& $70 \pm 0.3$\\
&Genesis (R)& $64\pm3$         & $65\pm3$ && $65\pm1$ & $42\pm1$ & $30\pm0.5$& $96\pm 0.6$ & $\bm{84 \pm 0.7}$\\
& Iodine    &  $70\pm9$  & $72\pm10$  & & $37\pm5$ & $ 62\pm4$ &$37\pm6$ &  $80\pm 8$  & $71 \pm 3$ \\
& Iodine (R)   & $35\pm2$         & $36\pm1$ && $17\pm2$ & $46\pm1$ & $61\pm2$& $75\pm 4$ & $65\pm 1$\\
\midrule
\multirow{6}{*}{Clevr6} &Monet (Att.)&   $\bm{46\pm5}$ & $\bm{48\pm5}$ && $22\pm4$ & $\bm{51\pm3}$ & $55\pm5$& $\bm{93\pm 0.4}$ & $\bm{68 \pm6}$\\
& Monet (Att.) (R) &   $40\pm9$ & $41\pm9$ && $13\pm5$ & $44\pm3$ & $61\pm8$& $\bm{93\pm 0.4}$ & $\bm{65 \pm5}$\\
&Monet (Dec.) &     $\bm{47\pm6}$ & $\bm{48\pm6}$ && $21\pm6$ & $\bm{50\pm4}$ & $55\pm5$& $90\pm 2$ & $65 \pm2$\\
&Monet (Dec.) (R) &   $40\pm1$ & $41\pm0.2$ && $13\pm0.6$ & $44\pm0.1$ & $60\pm0.6$& $92\pm 0.5$ & $\bm{69 \pm1}$\\
&Genesis	& $\bm{50\pm2}$    & $\bm{52\pm2}$&& $\bm{47\pm2}$& $39\pm2$&$\bm{47\pm0.9}$&$91\pm 0.4$& $65 \pm 3$\\
&Genesis (R)& $43\pm1$         & $45\pm2$ && $24\pm2$ & $21\pm2$ & $65\pm1$& $92\pm 0.2$ & $60 \pm 3$\\
\bottomrule
\end{tabular}
\end{sc}
\end{footnotesize}
\end{center}
\vskip -0.1in
\end{table*}
